The Robustness of Tether Friction in Non-idealized Terrains

Reduced traction limits the ability of mobile robotic systems to resist or apply large external loads, such as tugging a massive payload. One simple and versatile solution is to wrap a tether around naturally occurring objects to leverage the capstan effect and create exponentially-amplified holding forces. Experiments show that an idealized capstan model explains force amplification experienced on common irregular outdoor objects - trees, rocks, posts. Robust to variable environmental conditions, this exponential amplification method can harness single or multiple capstan objects, either in series or in parallel with a team of robots. This adaptability allows for a range of potential configurations especially useful for when objects cannot be fully encircled or gripped. These principles are demonstrated with mobile platforms to (1) control the lowering and arrest of a payload, (2) to achieve planar control of a payload, and (3) to act as an anchor point for a more massive platform to winch towards. We show the simple addition of a tether, wrapped around shallow stones in sand, amplifies holding force of a low-traction platform by up to 774x.

==> Harnessing the Environment - ArXiv (pre-RA Letters)/1intro.tex <==
\section{Introduction}

%\IEEEPARstart{M}{obile} 
%\IEEEPARstart 
%\subsection{Forceful mobile robotic systems}
%Mobile 
Mobile robotic systems enable tasks like remote exploration, automated construction, and search and rescue. Natural terrains and unstructured environments can consist of loose and slippery media such as sand, shale, detritus, snow, mud, and biofilm. These surfaces support only limited shear and frictional contact forces for locomotion and payload maneuvering. Therefore, small robots often require enhanced or specialized foot designs to improve contact conditions, like %. Instead of focusing on improving the traction of a single robot through end effector specializations, such as 
treads, adhesives, or spines. Instead, we explore how to create forceful robot systems even when traction remains low. As depicted in Fig. \ref{fig:concept}, %the technique harnesses 
tethers connecting multiple robots are purposefully wrapped %these tethers 
around terrain features available in the environment. %, like trees, rocks, and poles. 
 By taking advantage of fixed anchors, tether-world friction supports exponential amplification of ground traction forces and the effective load holding capacity of simple lightweight mobile robots.


\subsection{Background: Tethered robots for payload manipulation}
Prior work demonstrates how tethered teams of robots manipulate payloads \cite{estrada_forceful_2018,christensen_lets_2016} and function as exploratory agents tethered to a “mother-ship” \cite{mcgarey_system_2016, stefanini_tether_2018}. Systems overcome obstacles in irregular environments using robot-robot cooperation through pushing \cite{mcpherson_team-based_2019, deshpande_methodology_2009} and exploiting tethers \cite{fukushima_development_2001,asano_tethered_2010, kitai_proposal_2005}. Tethers enable the pulling of other robots or may act as static lines to provide paths for a locomotion network of spider-like robots \cite{shoval_design_1999, hao_design_2011}. Tethered demonstrations include pair-wise cooperation for stair climbing \cite{casarez_step_2016}, mapping extremely steep terrain \cite{mcgarey_developing_2018}, descending over steep edges \cite{bares_dante_1999,mumm_planetary_2004}, and larger scale ascent and descent with a tether \cite{schempf_self-rappelling_2009}. Single agent systems include a rover capable of tugging a sled on sand \cite{fernandez_tail-based_2021}, or a robot with “reaching arms” that moves a load when pulling in tension \cite{schneider2021reachbot}. %For tethered navigation in unstructured terrain, one work \cite{mcgarey_tslam_2017} provides tethered simultaneous localization and mapping (TSLAM) that estimates the location of tether-object contact points. 

\begin{figure}[t]

    \centering
    \includegraphics[width=1\columnwidth]{figure/fig1.png}
    \setlength{\abovecaptionskip}{-10pt}
    \caption{ \textbf{Capstan-enabled maneuvers} Example exploitation of natural capstans for robotic missions on low-traction substrates are demonstrated. 
    %Selected capstan objects range from single objects to numerous objects and from environment-provided objects to man-made infrastructure. 
    Capstan objects are shown utilized in single (top), serial (middle), and parallel (bottom) configurations. Robotic teamwork, target transport, and multi-millibot or swarm scaling modes, respectively, are all enabled through capstan amplification. Photo credits: (top) H.S. Stuart, (middle) R. Henrik Nilsson, CC BY-SA 4.0, (bottom) Jar.ciurus, CC BY-SA 3.0 PL.
    }
    \label{fig:concept}
    \vspace{-6mm}
\end{figure}

These works assume robust attachment or traction with the world, achieved through specialized gripping or anchoring mechanisms \cite{estrada_forceful_2018,christensen_lets_2016,fernandez_tail-based_2021,schneider2021reachbot}, making an agent massive enough to be assumed unmovable \cite{mcgarey_system_2016}, or manually pre-deploying secure anchor points by researchers \cite{kitai_proposal_2005}. Applications outside of these specific scenarios warrant new robust and more generalized lightweight methods for the mobile creation of secure anchor points on the fly in the field. 

Many natural environments contain effectively fixed objects, such as trees or rocks. For tethered navigation in unstructured terrain, one work \cite{mcgarey_tslam_2017} provides tethered simultaneous localization and mapping (TSLAM) that estimates the location of tether-object contact points. Past literature \cite{stefanini_tether_2018,kumar_entanglement_2007,a_specian_friction_2015} cites these 
terrain features
%naturally occurring obstacles
as a primary disadvantage of tethered teams due to tether abrasion, unpredictable snagging, and tangling. In contrast, we leverage this tether-environment contact and propose to use these 
terrain
%naturally occurring 
features to exponentially amplify the available resistive traction forces through the capstan effect. 

Despite the long-term establishment of capstans throughout history, the application to robotics is first mentioned in work by Augugliaro et al\cite{augugliaro_building_2013}, in which aerial vehicles are used to build tensile structures such as footbridges. This work focuses on the planning and execution of knots and wraps around indoor structures, expanded upon by Segal et al \cite{segal_method_2021}, who extend the method to natural features like trees. They do not characterize the variability or predictability of the simple capstan equation on natural objects like rocks and trees, nor do they discuss the amplification of contact forces as applied by mobile ground vehicles for flexible payload manipulation. 
Although complex models that account for tendon extensibility \cite{d_kuhm_fabric_2014} or radius and irregularity of capstan cylinder \cite{howell_friction_1954,jayawardana_capstan_2021} exist for controlled laboratory settings, there remains an opportunity to characterize the robustness of this mechanism on real-world terrains. % for robotic payload manipulation with mobile ground vehicles, as we do in the present work. 
\emph{We present the first study that verifies whether conventional formulations provide practical estimates for robot applications in the field, even with partial wraps on irregular natural capstan objects}.


\subsection{Overview}
Sec. \ref{sec:model} summarizes idealized tether friction amplification behavior. We contrast different robotic anchoring technologies with capstan amplification using scaling arguments for natural objects.
In Sec. \ref{sec:results}, we explore the applicability of the generalized capstan equation to multi-capstan systems in series, %and show that wrap angles are summed across multi-capstan wraps with equal µ, 
a previously unproven assumption. We then present %the first set of 
experiments characterizing tether friction on natural objects in the field. %, and find that the capstan equation provides useful estimates even on highly rugose and non-circular natural materials. 
We observe that capstan slip is often non-catastrophic and can further amplify holding force. %, due to substrate mounding and tether-object snagging. %In a laboratory experiment on granular media, a tether wrapped around two natural objects is capable of yielding an $A_F$ at failure of 774x and fails due to object upheaval, not tether slip. 
In Sec. \ref{sec:demo}, we illustrate these principles on robotic systems in both the laboratory and the field, % to \textit{(i)} serve as anchors for winching of a payload, \textit{(ii)} control lowering of a payload, and \textit{(iii)} control the planar manipulation of a payload via tethered agents in parallel. %\textit{(iv)} 
%As an demonstration of practical application in the field, a pair of agents then cooperate to %harnesses a capstan in a natural forest environment to 
%free the entrapped vehicle, which is 11x times the mass of the tether-deploying agent. 
and Sec. \ref{sec:discuss} provides a discussion on real-world tether deployment considerations. Sec. \ref{sec:conclusion} summarizes applications for future work.



\section{Harnessing the Capstan Effect}
\label{sec:model}

%Many natural environments contain effectively fixed objects, such as trees or rocks. Past literature \cite{stefanini_tether_2018,kumar_entanglement_2007,a_specian_friction_2015} cites these naturally occurring obstacles as a primary disadvantage of tethered teams due to tether abrasion, unpredictable snagging, and tangling. In contrast, we leverage this tether-environment contact and propose to use these naturally occurring features to exponentially amplify the available resistive traction forces through the capstan effect. 
Tether tension amplification factor, $A_F$, is the instantaneous ratio between load tension, $T$, and holding force, $T_0$, or that $A_F=T/T_0$. The capstan equation states that $A_F$ %at first instance of slip 
scales exponentially with both wrap angle, $\theta$, and the coefficient of friction between the tether and the capstan, $\mu$, or that $A_F=e^{\mu\theta}$. By harnessing the capstan effect, even lightweight machines on materials with low surface attachment strength, or low $T_0$, can withstand tremendous pulling forces $T$. %This effect does not apply if $T_0=0$, as $A_F$ would become 0, assuming negligible tether mass. Thus, t
%Since the tether friction amplifies the tractive ability of an existing system, astrictive/enveloping methods can still be used to create strong attachment forces by the agent, which generate even greater force abilities when coupled with capstan amplification. 

As shown in Fig. 1, we envision small, lightweight, terrestrial mobile robots in single or multi-robot systems, capable of resisting large loads by applying capstan amplification on a range of geologic, living, or built features. A tethered team exploiting capstans can \textit{(i)} pull payloads, \textit{(ii)} lower payloads, and \textit{(iii)} achieve multi-dimensional motion. Additionally, the tethers can be \textit{(i)} wrapped around a single feature, \textit{(ii)} wrapped around multiple features, or \textit{(iii)} applied to multiple mobile robots in parallel. 
% not sure ``serial'' is best word here
For systems with serial capstan wraps, we expect that, within the traditional capstan equation, the product of $\mu$ and $\theta$ may be summed within the exponential: $T = T_0e^{\sum_{i} \mu_i \theta_i }$. %This assumption is validated in Results: \textit{Scaling of capstans}. 
For systems with multiple mobile agents applying capstan wraps, individual tension vectors may be summed: $\vec{T} = \sum_{j} T_{0,j}e^{\mu_j \theta_j } \vec{t_j}$, where $\vec{t_j}$ represents the unit direction vector of each agent's tether.
%We hypothesize that these conventional capstan equations describe tension amplification even in natural environments. %, across these varied scenarios. 
%Although complex models that account for tendon extensibility \cite{d_kuhm_fabric_2014} or radius and irregularity of capstan cylinder \cite{howell_friction_1954,jayawardana_capstan_2021} exist for controlled laboratory settings, we present the first study that verifies whether these conventional formulations provide practical estimates for robot applications in the field, even on highly irregular natural capstan objects.



\begin{figure}[t]

    \centering
    \includegraphics[width=1\linewidth]{figure/fig2.png}
    \setlength{\abovecaptionskip}{-10pt}
    \caption{\textbf{Comparison to robotic attachment methods.} Comparison of properties of various attachment modes frequently used by robots. 
    %Traditionally, surface gripping methods' strength scales with contacting surface area and the gripped surface's strength  
    %\cite{yano_development_1997,carpenter_rotary_2016,jiang_stochastic_2018}. 
    %Envelopment methods, such as natural capstans, present a unique opportunity to leverage the compressive radial strength of materials rather than the comparatively weaker surface shear or tensile strengths. The capstan effect enables a lightweight tether to amplify tension forces on large and sturdy objects. 
    %Values of failure force vary within object class (tree, rock) and species. Forces calculated based on average redwood tree dimensions from Fig. \ref{fig:muinnature} using strength values from \cite{green_wood_2001}. 
    The simplified capstan effect amplifies tendon tension $T$ exponentially with wrap angle $\theta$ and friction coefficient $\mu$.  Tension scales linearly with normal force $N$ and is independent of local radius $R$.
    }
    \label{fig:comparison}
    \vspace{-6mm}
\end{figure}

\subsection{Comparison with other anchoring modes}

As shown in Fig. 2, we distinguish \textit{capstan amplification} from \textit{surface attachment} and \textit{enveloping grasps}. % in tether anchoring. 
There is a rich history of \textit{surface attachment} mechanism design research, % like treads and grippers to strengthen shear limits, 
including %for more forceful maneuvers. Such mechanisms include, but are not limited to, 
spines \cite{jiang_stochastic_2018},  %\cite{carpenter_rotary_2016, jiang_stochastic_2018, asbeck_designing_2012}, 
suction \cite{yano_development_1997}, electrostatics \cite{prahlad_electroadhesive_2008}, and adhesives \cite{wang_large-payload_2013, hawkes_geckos_2013}. These astrictive grasping mechanisms develop high shear and normal forces at the surface, and thus fail when the surface material fails. They also tend to be specialized for specific surfaces; for example, present gecko-inspired adhesives perform exceptionally on clean polished surfaces, but reduce performance on rugose or dirty surfaces. \textit{Enveloping grasps} overcome these limitations by compressing the surface material, but require that the robotic gripper find features small enough to wrap around. %, yet strong enough to resist external forces. 
Recent examples include a biomimetic robot for bird-like perching in arboreal environments \cite{roderick_bird-inspired_nodate}, autonomous perching by quadrotors on cylindrical objects \cite{thomas_visual_2016}, and a plant tendril-like robot that coils around branches and stiffens to create an envelopment grasp \cite{meder_plant_2022}.

In contrast, \textit{capstan amplification} with a tether allows for anchoring on objects of widely varying sizes and surface properties with greater strength. The capstan amplification effect is especially robust in its ability to exploit anchor objects with a variety of non-ideal surfaces, such as wet, crumbling, or rough surface conditions. Maximum object size is limited primarily by the length of tether available. At a sufficient wrap angle, object failure can occur under radial compression; in the case of a tree or rock, radial compression requires on the order of $10^4$ N or $10^6$ N of force, respectively \cite{green_wood_2001}\cite{wyllie_chapter_1996}, providing between two and five orders of magnitude more force than surface failure. 
On well-anchored  objects, i.e. force of upheaval is greater than maneuver force, tendon strength likely limits maximum loading ability before object failure occurs. Since the tether friction amplifies the tractive ability of an existing system, surface/enveloping methods can couple with capstans to create even stronger attachment forces by an agent. %, which generate even greater force abilities when coupled with capstan amplification. 

All attachment modes may fail if the feature itself moves: a tree is uprooted from the soil or a boulder slides along the ground. These upheaval forces vary with the object’s mass and ground interaction forces. For young trees and smaller rocks, upheaval forces range from tens to hundreds of Newtons, while for strongly rooted older trees and large boulders these forces reach the order of kN or larger \cite{lindroos_forces_2010}. %In high-force applications, it becomes pertinent to select objects based on resistance to upheaval. %As such, assuming the robot applying the tether is able to achieve sufficient wrapping, failure of a capstan attachment requires several orders of magnitude greater force than surface attachment modes, which will sooner exhibit shear or tensile failure of the substrate or mechanism.



%\subsection{Overview}

%In the following sections, we present findings on the capstan effect's applicability to irregular objects and multi-object systems, then apply the findings to demonstrate forceful robotic maneuvers. 
% In Sec. \ref{sec:results}, we explore the applicability of the generalized capstan equation to multi-capstan systems in series, and show that wrap angles are summed across multi-capstan wraps with equal µ, a previously unproven assumption. We then present the first set of experiments characterizing the capstan effect on natural objects in the field, and find that the capstan equation provides useful estimates even on rugose and non-circular natural materials. We also observe that capstan slip is often non-catastrophic due to substrate mounding and tether-object snagging. 
% %In a laboratory experiment on granular media, a tether wrapped around two natural objects is capable of yielding an $A_F$ at failure of 774x and fails due to object upheaval, not tether slip. 
% In Sec. \ref{sec:demo}, these principles are then illustrated with capstans in a laboratory setting to \textit{(i)} serve as anchors for winching of a payload, \textit{(ii)} control lowering of a payload, and \textit{(iii)} control the planar manipulation of a payload via tethered agents in parallel. %\textit{(iv)} 
% As an demonstration of practical application in the field, a pair of agents then cooperate to %harnesses a capstan in a natural forest environment to 
% free the entrapped vehicle, which is 11x times the mass of the tether-deploying agent. Sec. \ref{sec:discuss} provides a discussion on tether deployment considerations.


















%Example Figure:
    

%\begin{figure}[t]
    %\centering    
    %\vspace{4mm}
    %\includegraphics[width=0.8\columnwidth]{figure/animals2.png}
    %\caption{%A number of organisms demonstrate different types of underground burrowing. 
    %There is a growing body of work on the design of bioinspired burrowing machines and robots. Pictured are three prominent recent examples of mechanisms and subsequent behaviors inspired by plant roots \cite{del_dottore_circumnutations_2016}, razor clams \cite{winter_razor_2014} and the sandfish lizard \cite{maladen_undulatory_2011}.  }
    %\label{fig:review}
%\end{figure}
%\begin{figure}[t]
    %\vspace{2mm}
   % \centering
   % \includegraphics[width=1\linewidth]{figure/conceptImage6.png}
   % \caption{ \textbf{Proposed 3D RFT methodology.} %\textbf{(A)} 
   % A visual representation of the process for estimating intrusion forces using RFT, from planar force characterization to summing the forces on all discretized plate elements on a 3D body throughout its motion. % \textbf{(B1)} Depiction of Euler angles transformation of a surface element, and the resultant orientation of the bases in 3D.  An example total velocity is indicated. \textbf{(B2)} The same plate element is viewed along the ${\underline{e}_{1}}$ axis, resembling a 2D RFT analysis as analyzed in \cite{li_terradynamics_2013}. The velocity in this plane, $\underline{v}_{23}$, is indicated. \textbf{(B3)} The plate element is viewed along the ${\underline{e}_{2}}$ axis, along with the $\underline{v}_{1}$ component of velocity.   %\textbf{(C)} %The proposed 3D RFT method could be applied to a wide range of applications. For example, t
   % There is a growing body of work on the design of bioinspired burrowing machines and robots; pictured is the case study of a mechanism, and subsequent 3D motion behaviors, inspired by plant root circumnutation used in the present study to validate the proposed 3D RFT method (credits: \cite{del_dottore_circumnutations_2016}, United States Department of Agriculture). %are three prominent recent mechanisms and subsequent behaviors inspired by plant roots (credits: \cite{del_dottore_circumnutations_2016}, United States Department of Agriculture), razor clams (credits: \cite{winter_razor_2014}, Arne Hückelheim / CC BY-SA 3.0) and the sandfish lizard (credit: \cite{maladen_undulatory_2011}, Ding, et al. / CC BY 2.5). 
  % }
  %  \label{fig:concept}
%\end{figure}






==> Harnessing the Environment - ArXiv (pre-RA Letters)/3resultsanddiscussion.tex <==




\section{Experimentation of Variability}
\label{sec:results}

%\subsection{Force measurement method}

%\subsubsection{Force data collection}
In order to characterize $A_F$ for the scenarios throughout this Section, we %first procuring force data using 
use a Mark-10 Series 4 hand-held force gauge. % is utilized. 
Data is obtained by 
%The process of obtaining data involves first identifying
first quantifying the holding force on a given substrate of a 25-gram 3D printed plastic sled, weighed down by a 200-gram calibration weight. A tether is tied to both the sled and the force gauge, then pulled via the force gauge until the sled’s first instance of slip, at which peak force is recorded as $T_0$. This process is repeated to identify the tension required to induce tether slip at a certain wrap angle, $\theta$, by %with the intermediate step of 
first winding the tether around the capstan(s). %, then again pulling until the first sign of slip. 
Throughout each of these trials, we keep tether length, angle, and contact height constant. 
Unless specified, the tether used in all experiments is HERCULES Dyneema 1mm, a pre-braided and abrasion-resistant fishing line. 

\subsection{Scaling to multiple capstans}
An extension of the simple capstan equation to multi-capstan systems predicts equal forces for equal total wrap angles, regardless of the number of capstans involved, provided the friction coefficient is constant on all capstan objects. %We first construct a laboratory test bed to maintain consistent robot-substrate and tether-object contact conditions. % while procuring force data to assess the extension of the capstan effect to multi-capstan systems. 
As shown in Fig. 3, a laboratory test bed consists of four one-inch (25mm) diameter steel rods on a Radiata pine plywood platform. Each rod is wrapped in 180-grit sandpaper %or 3M gaffers tape 
to mimic a tether-rock %or tether-tree 
interface both in friction and abrasive qualities. The tether and sandpaper %or tape 
were replaced frequently to diminish changes in the coefficients of friction between worn surfaces. With this setup, the number of capstans, path of the tether, and wrap angles can all be varied.
The tether friction of each cylinder is individually measured with a 720-degree wrap. % is applied to a single cylinder in the experimental testbed, as in Fig. 3A1e. The corresponding $A_F$ at the first instance of slip is determined for each individual post, the wrap angle, materials, and $T_0$ constant. 
The variation between the highest and lowest $A_F$ is 32$\%$, with mean friction coefficient 0.6$\pm$0.1.


As shown in Fig. 3A1(a)-(j), we measure holding force amplification across different \textit{permutations of serial wraps}, %, using a weighted sled, force gauge, and metal rods (shown in Fig. 3B). These sequences of wraps 
representing total summed wrap angles of 360 or 720 %, and 900 
degrees across one, two, or four cylindrical rods. The resulting $A_F$ at first instance of slip is measured for 15 trials at each combination of conditions. %, is plotted in Fig. 3A2. 
In Fig. 3C, which represents data from 3A combined across all 720 and 360- degree trials, $A_F$ at slip is significantly higher for a single capstan wrap than in cases with multiple capstans in series, at 36$\%$ and 29$\%$ higher, respectively. %However, there is no statistically significant difference between two and four capstan wraps. 
Statistical significance is tested with %When identifying statistical significance between laboratory-tested wrapping combinations, 
a one-way ANOVA test %was performed 
followed by Tukey’s HSD.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figure/fig3.png}
    \setlength{\abovecaptionskip}{-10pt}
    \caption{ \textbf{Investigation of capstan effect across multiple capstans.} \textbf{(A1a-j)} All tested permutations of wrap angles summing to 360, 720, and 900 degrees, corresponding to data in (C). 
    %\textbf{(A2)} Mean force amplification $A_F$ at slip for each wrap permutation in (A1), with error bars representing standard deviation. 
    \textbf{(B)} Experimental setup for laboratory capstan testing
    %, in which the capstan objects, tether, holding force (sled), and load (force gauge) are denoted. 
    \textbf{(C)} Mean $A_F$ at slip produced as a function of number of capstans. 
    %Dark blue bars represent combinations of wraps which sum to 720 degrees while red bars represent combinations which sum to 360 degrees.
    Statistical significance is indicated with ** corresponding to p $<$ 0.005.  
    \textbf{(D1)} $A_F$ for the various permutations of capstan material order presented in \textbf{(D2)}. S and T abbreviate sandpaper and tape, their friction coefficients $\mu_S$ and $\mu_T$. * corresponds to p $<$ 0.05.
    }
    \vspace{-6mm}
    \label{fig:no. capstans}
\end{figure}

The discrepancy in $A_F$ observed between one and multi-capstan wraps can be explained by the sensitivity of the capstan equation to small changes in friction coefficient, $\mu$, at large wrap angles. According to the capstan equation, differentiating $A_F$ with respect to both $\mu$ and $\theta$ yields $\frac{d}{d\mu} A_F = \theta e^{\mu\theta}$ and $\frac{d}{d\theta} A_F = \mu e^{\mu\theta}$. The typical $\mu$ is on the order of 0.25 - 0.5 for natural objects and 0.24 for the tape used on the lab testbed. Typical wrap angles for practical applications will be significantly larger than 0.5 radians or $\sim$30 degrees. Thus, we note that $\theta > \mu$ and ergo $\frac{d}{d\mu} A_F > \frac{d}{d\theta} A_F$. 
For a single capstan wrap, and assuming a typical $\mu$ of 0.3 and $A_F$ of 10, a 1\% change in $\theta$ will result in a 3.7\% change in $A_F$. However, for an $A_F$ of 10 with a wrap angle of 720 degrees, a 1\% change in $\mu$ will result in a 125\% change in $A_F$. 
As wrap angles increase, $A_F$ becomes more sensitive to small changes in $\mu$. 
%For this example of wrap angle and friction, $A_F$ will be over 30 times more sensitive to changes in $\mu$ than changes in $\theta$. 
%As the magnitude of wrap angle on any individual capstan is higher for a single capstan than those distributed over multiple capstans, slight variations in $\mu$ have large consequences on the resultant $A_F$. 
%Single capstan wraps are more likely to see a wide variation in $A_F$, and possibly altered mean $A_F$, over equivalent $\theta$ multi-capstan wraps. 

We test the role of variable friction (Fig. 3D) by placing a lower friction capstan material (3M gaffers tape), %,  $\mu_T= 0.24\pm0.1$)
among a 720-degree wrap containing two other capstans of a higher friction material (180-grit sandpaper).
%$\mu_S= 0.60\pm0.13$) 
The sequence which places the lowest friction capstan closest to the holding force (Tape Sandpaper Sandpaper or TSS) demonstrates the lowest mean force amplification. Likewise, placing the lowest friction capstan closest to the load (SST) results in the highest mean force amplification. We observe statistical significance between these two extreme scenarios, but not when they are compared with the intermediate scenario (STS). Given our friction sensitivity analysis and large variation observed, $A_F$ at slip is assumed to be independent of the sequence of $\mu$. 

As expected, this data supports the idea that the product of $\mu$ and $\theta$ may be summed within the exponential for multi-capstan wraps with varying friction. 
In practice, multiple capstans are preferred over a single capstan; % semi-colon instead of comma(?) maybe split sentence
when objects present a variety of friction coefficients that are difficult to predict accurately, 
multiple capstans provide an averaging effect that is insensitive to object order. However, if the highest friction object is identifiable, then a single capstan utilizing that one object supports higher tether tensions for a given wrap angle.
%Other complicated environmental factors related to the ground conditions and tether snagging interactions contribute significantly to force amplification as well, and we explore these contributions in more depth in the section \textit{Non-catastrophic failure}.




\subsection{Capstans in the natural environment}


We measure the amplification factor of different outdoor objects – geologic, living, and built – in order to provide the first investigation of whether the simple capstan effect holds true across a variety of real objects in the field. We select London planetrees (n=2), a palm tree, rocks (n=4), a lamp post, a fire hydrant, and redwood trees (n=10) at the University of California at Berkeley campus to provide a variety of common local objects. %We use the same sled and force gauge as in Fig. 3 and wrap around one object at a time. 
For each object, we wrap the tether to 90, 180, 270, 360 or 450 degrees and record the resulting tension required to induce tether slip; each condition is repeated five times. Snags on the bark are avoided during tether application. 
$A_F$ at slip is computed across these trials using a $T_0$ value collected over five independent trials at the location of each object, without any object wrapping or tether friction. 

\begin{figure}[t!]
    \includegraphics[width=1\linewidth]{figure/fig4_new.png}
    \setlength{\abovecaptionskip}{-10pt}
    \caption{ \textbf{Characterization of friction for various natural capstans.} \textbf{(A1) - (A6)} Images of capstan objects, with friction coefficient fit to the means of 5 trials at each wrap angle. Wrapped tether location indicated with a dashed red line. Standard deviation is reported for multi-object data sets. Plots below each image show the measured mean and standard deviation tension amplification at each wrap angle with a dashed curve representing the fit $\mu$. \textbf{(B1)} Tension amplification measured across 10 redwoods and 5 different wrap angles, corresponding to 50 data points at each wrap angle, described by the box plots. The red shaded region indicates the 95\% confidence interval on the friction coefficient fit to all data points. The lowest black line and gray region above indicates the lowest measured friction coefficient for wrap angles above 360 degrees.  \textbf{(B2)} Plot of fit friction coefficient for each redwood as a function of tree circumference, with a fit line that indicates a weak positive correlation. }
    \label{fig:muinnature}
    \vspace{-6mm}
\end{figure}

As reported in Fig. 4A1-6, the coefficient of friction µ in the capstan equation is treated as a fit parameter, and the exponential curve is fit to five data points using the MATLAB R2019b Curve Fitting toolbox. %An estimate of friction for each object is extracted from a best fit of the generalized capstan equation to the means of five trials at each wrap angle. The resulting estimated coefficients of friction are reported in Fig. 4A1-5, and images corresponding to each object are displayed. 
It should be noted that coefficients of friction may depend on the ever-changing wear, aging, abrasion, and interactions of particles sheared off of both the tether and capstan object over many trials; we reduce environmental variability by conducting experiments on days with similar conditions and replacing the tether between trials. Further, all data for each individual capstan object was gathered in one day. The coefficients of friction of the objects shown in Fig. 4A1-6 range from 0.26 for smooth bark to 0.5 for the fire hydrant. The $A_F$ versus wrap angle relationship of each of these objects follows an exponential trend matching the capstan effect, despite deviation from the idealized smooth and circular geometry, e.g., the redwood tree is highly rugose, and the rock is irregularly shaped.

We investigate intraspecies variation by comparing the 10 different \textit{Sequoia sempervirens} (coast redwoods) in order to inform expected performance of capstan amplification in specific environments; the current data set is particularly useful in a redwood forest. Coefficients of friction range from 0.336 to 0.466 with mean $\mu$= 0.38 and $\sigma$ = 0.04, as reported in Fig. 4B1. %Fig. 4B2 compiles data from all redwood trees, showing s
Shaded regions represent the fit and confidence bounds over all trees. %Based on this data set, w
We propose that an agent can estimate amplification factors, with an associated level of confidence, through visual classification of available object types alone, which is useful for planning maneuvers.

The idealized capstan equation neglects the shape and diameter of the capstan and amount of surface contact between the tether and capstan. Prior literature shows little effect of object radius on corresponding capstan force in the lab \cite{howell_friction_1954}. Circumferences of natural capstans of the \textit{Sequoia sempervirens} are estimated using strands of rope wrapped in an identical fashion to that in force experiments, and later measured against a tape measure. We check for diameter correlation across the \textit{Sequoia sempervirens} data set in Fig. 4B4, where we plot the mean calculated friction coefficients for each redwood tree as a function of its circumference. Only a weak positive correlation is present, largely supporting the diametral independence assumption for this species. The slight trend may be rooted in the rugosity of this species’ bark. Larger-radius natural objects provide a larger surface area, and thus increase the chance of imperfections and snag points on the tether that increase $A_F$. Younger redwood trees tend to have smoother bark and smaller trunk diameters. 

In the present work, we assume dry conditions. However, weather conditions may affect the friction coefficients of tether-object contact. We collect initial data on the experimental test bed (Fig. 3B); two different strings are wrapped in both dry and wet conditions around an object at 90-degree increments up to 450 degrees. The objects selected are a steel metal post, a post covered in tape as in Fig. 3, and a rock. We introduce dampness into the tether-object system via soaking the object and tether. Wetness did not consistently increase or decrease the coefficient of friction. For HERCULES Dyneema 1mm, the change in friction coefficient from dry to damp was +13.0\% for the tape post, -0.9\% for the metal post, and -1.5\% for the rock. For PTFE yarn, the changes were +5.6\%, +7.3\%, and +10.0\%.  %and never changed the friction coefficient by more than 13\%. 
Thus, environmental-capstan appears robust to moisture. %the objects being wet. 

%When visually examining the geometry across all objects in Fig. 4A1-6 and B1, data broadly matches the generalized capstan equation despite deviation from the idealized smooth and circular geometry, e.g., the redwood tree is highly rugose, and the rock is irregularly shaped.






\subsection{Exceeding the capstan effect: Non-catastrophic slip}

Once a system’s applied loading force exceeds the capstan-amplified holding force, slipping of the tether on the capstan occurs. In real-world applications, forces can increase after this onset of tether slip such that these capstan failures are not catastrophic for the maneuver. We observe that slip can \textit{(i)} induce geometric snagging of the tether on the capstan and \textit{(ii)} increase the $T_0$ by pulling the agent through the terrain.

As greater force is applied to a tether, it cinches, leading the tether to settle in local concavities on the capstan object. As slip occurs, the tether can further dig into capstan objects and enter a pinched position. As shown in Fig. 5A and 5B, the tether becomes pinned beneath bark features on a tree or within crevasses of a jagged rock. Snags can appear immediately upon loading or develop after tether slipping, yet Fig. 5A and 5B both show the case in which snagging occurs after initial slip. Snagging increases the amplification factor by approximately 3x in both cases shown. We hypothesize that the shear strength of the capstan-object’s surface correlates with snagging amplification factor, as a weak surface would shear off under snagging stresses. While an advantageous mechanism for increasing holding force, snagging is disadvantageous if the tethered agent is intended for repeatable use, as snagging can impede unwinding.

As an object is dragged across a loose substrate, particles gather on the leading surface over time, and this interaction increases the $T_0$ capabilities of the agent. Heterogeneous substrates, such as the mulch in Fig. 5A2, contain sticks and other particles that can build up resistance to an object dragged through the surface. As a result, stick-slip force variations of the holding agent increase; as seen in Fig. 5C2, the sliding force on mulch varies by 70$\%$ as compared with 38$\%$ on smooth plywood. In a more homogeneous media, like sand, $T_0$ increases until granular resistive forces reach a steady state \cite{li_terradynamics_2013}. One pull test in a bed of granular media shows an increase of holding force by 33$\%$ due to sand mounding, as seen Fig. 5C3.

Each of the above phenomena compound to assist in arresting tether slip events. % by increasing the holding force in both natural and controlled environments. 
Robots may therefore operate close to capstan limits with low risk.
Future system designs may amplify these holding effects, for example by actively increasing mounding. % through body shape design. 
It must be noted that slip wears tethers, thus this modality can fail over time due to tether abrasion. 


%In natural environments, weather can introduce dampness into the system, which can effect the friction coefficient. While water can sometimes act as a lubricious layer, it was found in testing two strings on a metal post both wet and dry that...

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figure/fig5_new.png}
    \setlength{\abovecaptionskip}{-10pt}
    \caption{\textbf{Dynamic slipping of capstan-tether system.} 
    \textbf{(A1)} A tether wrapped around a redwood tree is manually pulled until slip and continued to be pulled for approximately 10 seconds. $A_F$ over time is plotted. 
    % During slipping, a snag develops within the bark, resulting in a threefold amplification in force.
    \textbf{(A2)} Experimental setup for redwood tree snagging, including a weighted sled ($T_0$), handheld force gauge ($T$), and a 360 degree wrap of the tree. \textbf{(B1)} A tether wrapped around a rock is pulled for 12 seconds after initial slip and $A_F$ over time is plotted. \textbf{(B2)}  Experimental setup for rock snagging data. \textbf{(C1)} Experimental setup for recording slip-stick and mounding phenomena, in which holding force is measured directly without capstan amplification. \textbf{(C2)} A sled is dragged across a heterogeneous and homogeneous substrate, experiencing variation in force required to promote motion. \textbf{(C3)} A sled dragged through one meter of MARS90 regolith simulant shows a gradual increase and subsequent leveling of force required to slip over time.
     }
    \label{fig:failuremodes}
    \vspace{-6mm}
\end{figure}


\section{Robotic Demonstration}
\label{sec:demo}

For robotic demonstrations, we use a MiniRHex as a representative small-scale tether-deploying agent. This cockroach-inspired robot employs six semi-compliant, 360-degree-rotating semicircular ``C-shaped'' legs shown to overcome loose natural terrain \cite{barragan_minirhex_2018} (weighs .425 kg and measures .19m long by .10m wide by .10m tall). %Other agents could replace the MiniRHex in other systems and applications. 
%\subsection{Robotic System}
%A representative prototype consists of a tether-deploying agent and winching payload. The stand-in agent, MiniRHex, an open-source code and design robotic platform %created by the CMU Robomechanics Lab 
%\cite{barragan_minirhex_2018}
A separate payload winching platform uses a %structure is an Arduino-controlled, 
75:1 geared brushed DC motor coupled to a spool for reeling and retaining the tether, affixed to an acrylic sheet. This platform is then attached to three separate bases: caster wheels for hard surfaces, a sled for granular surface, or a rover. %affixed to an acrylic sheet with caster wheels. The dolly %structure 
%weighs 1.24 kg unweighted and 3.34 kg weighted. %, seen in Fig. 6. 
The caster and sled dollys weigh 3.34 kg  and 2.62 kg, respectively.
%This same acrylic assembly is seen fixed atop a representative rover in Fig. 6. 
The rover, from \cite{cao_mobility_2021}, is 4.8 kg, 0.30m long by 0.30m wide by 0.15m tall. %, and designed for granular media %using different rotational speeds of the front and back tires 
%A detailed view of MiniRHex, the dolly structure, and rover are presented in supplementary Fig. S2. 

%\hs{Videos of demonstrations are provided in supplemental material.}


\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figure/fig6.png}
    \setlength{\abovecaptionskip}{-10pt}
    \caption{ \textbf{Visual summary of laboratory robotic demonstrations} \textbf{(A1)} MiniRHex in granular media applies partial tether wraps on two rock capstan objects. A dolly equipped with a winch then winches towards the anchored MiniRHex. \textbf{(A2)} Motion capture data over time of the rocks, dolly, and MiniRHex. \textbf{(B1)} The same two rock capstans as in (A1) are wrapped to 360 degrees and pulled until failure. 
    %A sled acts as the holding force and handheld force gauge measures load.  
    %When loaded to failure, the rock closest to the load is dislodged before the sled slips on the media.
    \textbf{(B2)} $A_F$ over time is plotted, demonstrating a peak $A_F$ of 774. \textbf{(C)} Before applying capstan wraps, a mass tethered to MiniRHex pulls it off of the platform. MiniRHex demonstrates, with the use of a tether-wrapped capstan object, the ability to control the lowering and arresting of this same mass. \textbf{(D)} Two MiniRHex robots demonstrate their ability to apply tethers on rectangular posts to allow varied planar motion of a weighted dolly.}
    \label{fig:demos}
    \vspace{-6mm}
\end{figure}





\subsection{Laboratory demonstration}

Fig. 6 presents a summary of laboratory robotic demonstrations mirroring the modalities presented in Fig. 1. %Fig. 7 then shows the application of this method in the field. Supplemental videos (Movies S1-5) present footage of all demonstrations. %The representative rover, dolly, and deployment of the MiniRHex are merely for demonstration purposes.

In Fig. 6A1, we demonstrate tethered payload locomotion in a laboratory environment containing a bed of granular media and two rock capstan objects.  %(see also Movie S4). 
MiniRHex, in this low-traction environment, applies partial wraps of tether around two rocks, then acts as an anchor for the weighted dolly, 8x heavier than MiniRHex, to winch itself forward. In Fig. 6A2, the motion capture data from the granular media demonstration shows that, after the winch begins to pull on the tether, neither MiniRHex nor the rock capstans move. For the same two rock capstan objects, we utilize an unweighted sled and handheld force gauge to test the tension amplification capabilities of this environment (shown in Fig. 6B1). The resulting tension force data, plotted over time in Fig. 6B2, reaches an $A_F$ of 774 before one of the rock capstans dislodges from the substrate. No visually observable tether slip occurs during this trial.

In Fig. 6C, we affix a mass and tether to a MiniRHex robot in order to demonstrate controlled target transport load lowering. %(see also Movie S2). 
Before applying capstan wraps, the mass overcomes the static friction force between MiniRHex and the platform, and MiniRHex is pulled off the platform. After applying two wraps around a single capstan, MiniRHex then precisely controls the lowering and arresting of the motion of the same mass by either walking backwards or stopping, respectively.

In Fig. 6D, two MiniRHex’s tethered to the same weighted dolly apply tether wraps on two separate rectangular posts, which allows controlled planar motion of the dolly through two separately controlled on-board winches. % (see also Movie S3). 
We demonstrate that the dolly is able to utilize its winches individually for locomotion towards a single agent’s capstan object, or simultaneously to locomote in a direction between the two objects. The right tether snags under the table leg utilized in the lab, while the left tether does not.
These principles also translate into unstructured outdoor environments.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figure/Fig8.png}
    \setlength{\abovecaptionskip}{-10pt}
    \caption{ \textbf{Visual summary of sequential capstan maneuvers} MiniRHex applies partial wraps to two buckets to act as anchor for the dolly to winch towards. MiniRHex then unwraps the partial wraps and moves to wrap on a new capstan object, allowing the dolly to maneuver to the desired area.
    }
    \label{fig:Sequence}
    \vspace{-6mm}
\end{figure}

%[Statement needed about why this is distinct from prior demos]. 
In Fig. \ref{fig:Sequence}, the dolly is now transported around an obstructive wall through multiple steps. This sequential task demonstrates the benefit of leveraging partial wraps on multiple capstan objects. % Two benefits of using partial wraps around multiple objects include use for (1) constrained spaces, where an object cannot be encircled, and (2) sequential tasks, by easing reversibility and redeployment of the same tether multiple times. 
 In the first step of the sequence, MiniRHex (Fig. 7A) applies low-angle partial wraps on two sand buckets with 180-grit sandpaper, used to mimic rock-tether contact. Multiple partial wraps are especially useful in this constrained space, where the MiniRHex is unable to fully encircle the buckets. The dolly then winches until located in a desirable position for the next maneuver. In Fig. 7B, MiniRHex then unwraps from the two buckets and applies a new wrap to the metal post. Once again, partial wraps provide an advantage, as opposed to full wraps or knots, because the tether path is reversed and re-applied elsewhere, without tangling. The dolly then winches a second time, moving to the desired location.

\subsection{Field demonstration}

In Fig. 8, a wheeled rover, stuck on a branch and unable to locomote, deploys a MiniRHex robot to apply a shared tether around an adjacent redwood tree. % (see also Movie S5). 
The MiniRHex successfully applies an approximately 360-degree wrap angle on the tree. The terrain consists of detritus, loose dirt and pine needles, yet the capstan-amplified holding force provides an anchor for the rover’s winch. The winch successfully frees the rover, which is 11x heavier than MiniRHex, from its stuck position. In this demonstration, slip occurs between the tree and tether, and the MiniRHex robot slips and tips over as the rover winches toward it. In a demonstration of non-catastrophic slipping, the maneuver succeeds, allowing the rover to %thereafter make forward progress after overcoming 
%overcome the obstacle anyway.	
free itself.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/fig7.png}
    \setlength{\abovecaptionskip}{0pt}
    \caption{ \textbf{Visual summary of outdoor robotic demonstration}  MiniRHex in an outdoor environment applies its tether to act as an anchor point for a stuck rover, weighing over ten times its mass, to winch towards.}
    \label{fig:Roverstuck}
    \vspace{-6mm}
\end{figure}


\section{Discussion}
\label{sec:discuss}

Despite the variation of natural objects and tether configurations, we find that the idealized capstan equation matches experimental data from the field. Tether slip failure in capstan amplification is also not necessarily catastrophic, providing opportunities for successful maneuvering despite operating near the amplification factor limit. In addition, we show that harnessing the capstan effect across multiple objects provides advantages, including for maneuver reversibility. 

%\todo{I'd consider putting your new moisture test results in the Discussion, because I feel that it is evidence to support further investigation in the future. Also, it doesn't fit nicely into any of the sections in III as-is.}

%Robots can use natural capstans in unstructured environments as a way to bolster existing tractive force, with the addition of a tether attached to a payload or payload-winching agent. Despite the variation of objects that can act as a capstan, we find that the simple capstan equation matches with varied experiments’ data, both in the lab and the field. We have specifically demonstrated this phenomenon on small-scale systems, without the addition of dedicated mechanisms for \textit{surface attachment} or \textit{enveloping grasping}, in order to highlight the potential simplicity of this force amplifying method. Tether slip failure in capstan amplification is also not necessarily catastrophic, providing opportunities for successful maneuvering despite operating near the amplification factor limit.

%In this section, we discuss the implication of our study for real-world systems, and for applications like search and rescue and exploration of unknown environments. Assumptions and potential limitations of this work can inform system design and deployment decisions that employ this force amplification method in future work.
 
%\subsection{Tether Deployment Considerations}

%\hs{Investigation into submerged environments will be a part of future work.} 

\subsection{Planning and executing tether deployment}

%\todo{Summarize what we can take away from our present work!, e.g. is multi or single capstan preferred based on friction variability, might you target objects or terrains that will have non-catastrophic failure? How to use the characterization from 4B1 to guide safety factor in planning, etc. Guidelines for human teleoperators \textbf{directly} from our work.}

Tether deployment %on
around natural capstans assumes the presence of suitable objects for wrapping, and %Many environments provide a wide variety of possible options; 
Fig. 4 yields insight into the variety of usable objects on the UC Berkeley campus and a redwood forest. Less obvious surfaces for capstan amplification include bushes, curved cliff walls, and even buildings, assuming an ability to deploy such a long tether. The minimum acceptable size for a %required for a 
capstan object is a function of the radius of curvature of the tether. % and the radius of the tether itself. %In this work, object diameters are at least 1 order of magnitude larger than the tether diameter.
%\todo{Wire effect future work.}

%Environments with sparse objects can still enable single-capstan engagement, while environments with dense objects allow for more options as to the utilization of multiple capstan objects. 
%Dispersing engagement across multiple objects has the potential to reduce the external loads experienced by any single object, however it can also increase the external load on an object by up to a factor of two in disadvantageous layouts as compared with the single-capstan case. Advantageous tether deployment can mitigate the risk of object upheaval.


We envision generating a library of common capstan behaviors between different tethers and field objects across more expansive environments in future work. Characterizations, like that of redwood trees in Fig. \ref{fig:muinnature}B1, can guide path planning. The lowest measured friction coefficient and 95\% confidence interval represent factor of safety bounds for safety-critical and less dangerous maneuvers, respectively. These factors of safety then inform minimum required wrap angles for an operation. Further path planning and active sensing strategies%within varied environments
, in order to optimize the strength of multi-capstan systems, is a topic of future work. For example, risk of capstan object upheaval can be mitigated by advantageously dispersing the tether to multiple capstans to decrease the objects' individually-experienced external force.

The physical deployment of a tether, being dragged around an object, as in this work, is limited by the friction of the sliding tether and maximum pulling force of the tether-deploying agent. This problem can be mitigated if the agent uses a lightweight tether and overshoots, or runs past, the desired capstan object in order to begin its wrap with excess slack tether on the ground. Future work will investigate tether-deploying agents that can unspool tether locally during deployment to reduce tether-environment sliding, 
%in concept like 
conceptually similar to tip-growing vines \cite{hawkes_soft_2017}, in order to engage with more objects or objects that are further apart. 


\subsection{Entanglement and reversibility}

Entanglement can occur during the deployment of tethers around capstan objects, and affects both the strength of the maneuver and the ability to reverse tether deployment. For example, when entanglement occurs, functions like lowering the payload in Fig. \ref{fig:demos}C can no longer be achieved. Tethers, when deployed in a slack state first, have a propensity to self-entangle when cinched, especially at high wrap angles. Whenever the tether-deploying agent must cross over or under the portion of tether, % connected to the distal agent. T
%this presents additional possibility for an entanglement between the tether-deploying agent and tether
it can also become entangled, such as hooking on a leg. When robot-tether entanglement occurs, the system enters a lasso- or knot-like envelopment grasp. %, and strength is no longer dictated by the capstan effect between the tether and capstan object. 
After a maneuver is completed, entangled tether may need to be cut free and left behind, so tangles should be avoided if reversibility and reusability are desired. %At each full 360-degree wrap increment around a single object, 
To avoid this circumstance, a distribution of partial wraps among multiple objects eases unwinding, especially if the tether never crosses its own path, as in Fig. 3A-d, \ref{fig:demos}A1 and \ref{fig:Sequence}. While removable knots present an option for reversible strong attachment, %capstan force amplification 
tether friction remains preferable for simplicity and necessary either for objects that cannot be encircled or for controlled sliding as in Fig. \ref{fig:demos}C.% when simplicity of wrapping and unwrapping are paramount. 


\section{Conclusion}
\label{sec:conclusion}

Mobile robots can use natural capstans in unstructured environments as a way to bolster existing tractive force and achieve manipulations, with the addition of a tether attached to a payload or payload-winching agent. 
%Despite the variation of natural objects that can act as a capstan, we find that the idealized capstan equation describes experimental data from the field. Tether slip failure in capstan amplification is also not necessarily catastrophic, providing opportunities for successful maneuvering despite operating near the amplification factor limit. In addition, we show that harnessing the capstan effect provides advantages, as opposed to knots, for maneuver reversibility. 
We specifically demonstrate features of this technique on a small-scale mobile system not optimized for forceful manipulation %, nor with the addition of dedicated mechanisms for \textit{surface attachment} or \textit{enveloping grasping}, 
in order to highlight
the high load handling capability provided
%what's possible 
with the simple addition of a tether and winch. This work therefore motivates the design and control of more specialized tethered systems that harness the capstan effect for specific applications. %the potential simplicity of this force amplifying method. 


\subsection{Future work: Applications}

%Utilizing capstan amplification yields potential to strengthen tethered robot teams for a wide range of potential applications. 
Equipped with a winch, urban search and rescue robots and remote explorers can use on-board deployable lightweight robots to traverse terrains that were previously unreachable, or to save a rover that has become stuck. Specialized lightweight robots could explore ahead, climbing steep inclinations, traversing loose substrates, or across unpredictable terrain, then act as anchor for a more massive robot or payload to winch itself across the obstruction. These same deployable robots could apply tethers near an excavation site, helping to move or lower massive raw material.
%resources. %A team of tethered agents could allow for 2D control of payloads through unpredictable environments. 
We expect that a variety of systems that can deploy a tether, whether flying, grounded, or submerged, can cooperate to achieve forceful maneuvers by harnessing this technique. % New considerations for the planning, control and design of such systems will be dictated by the desired load magnitudes, maneuvers and environments.} %, as the capstan effect creates an exponential force amplification irrespective of the source of the forces.w

















